Input Influence Matrix Design for MIMO Discrete-Time Ultra-Local Model

Ultra-Local Models (ULM) have been applied to perform model-free control of nonlinear systems with unknown or partially known dynamics. Unfortunately, extending these methods to MIMO systems requires designing a dense input influence matrix which is challenging. This paper presents guidelines for designing an input influence matrix for discrete-time, control-affine MIMO systems using an ULM-based controller. This paper analyzes the case that uses ULM and a model-free control scheme: the H\"older-continuous Finite-Time Stable (FTS) control. By comparing the ULM with the actual system dynamics, the paper describes how to extract the input-dependent part from the lumped ULM dynamics and finds that the tracking and state estimation error are coupled. The stability of the ULM-FTS error dynamics is affected by the eigenvalues of the difference (defined by matrix multiplication) between the actual and designed input influence matrix. Finally, the paper shows that a wide range of input influence matrix designs can keep the ULM-FTS error dynamics (at least locally) asymptotically stable. A numerical simulation is included to verify the result. The analysis can also be extended to other ULM-based controllers.

==> method.tex <==
Supposing the input influence matrix $\mathcal{G}_k$ in output trajectory tracking control law \eqref{FTScontroller}  is unknown, we can formulate a constrained optimization problem to design the control input $u_k$ and the input influence matrix $\mathcal{G}_k$ concurrently. The finite-time stable tracking control law can be formulated as an equality constraints of a min norm controller:

\begin{equation}
    \begin{array}{c}
    \underset{\mathcal{G}_k, u_k}{\min} \|u_k\|_2^2 + w \|\mathcal{G}_k\|^2_{F} \\
    \mathcal{G}_k u_k=f_k \\
    % u_k \in \mathcal{U}, \mathcal{G}_k \in \mathcal{G} \\
    u_{\min} \le u_k \le u_{\max}, \\
    \|\mathcal{G}_{k} - \mathcal{G}_{k-1}\|_F\le L\|y_{k} - y_{k-1}\| \\
    sign(\mathcal{G}_{k}^{i,j})=s_{i,j}
    \end{array}
\end{equation}
where $w$ is a small positive weight to prevent $G_k$ from going to $0$. $u_{\min}$ and $u_{\max}$ are the lower and upper bounds of the control input. We also constrain the $\mathcal{G}_k$ to be Lipschitz continuous. Note that constraints on the sign of $\mathcal{G}_k$ is necessary. If we replace $\mathcal{G}_k$ with $-\mathcal{G}_k$, $-u_k$ then becomes the solution, which may not regulate the tracking error but amplifying it. 

TODO: We have to estimate the bounds of the tracking error here.
